Underwater 3D positioning on smart devices

The emergence of water-proof mobile and wearable devices (e.g., Garmin Descent and Apple Watch Ultra) designed for underwater activities like professional scuba diving, opens up opportunities for underwater networking and localization capabilities on these devices. Here, we present the first underwater acoustic positioning system for smart devices. Unlike conventional systems that use floating buoys as anchors at known locations, we design a system where a dive leader can compute the relative positions of all other divers, without any external infrastructure. Our intuition is that in a well-connected network of devices, if we compute the pairwise distances, we can determine the shape of the network topology. By incorporating orientation information about a single diver who is in the visual range of the leader device, we can then estimate the positions of all the remaining divers, even if they are not within sight. We address various practical problems including detecting erroneous distance estimates, addressing rotational and flipping ambiguities as well as designing a distributed timestamp protocol that scales linearly with the number of devices. Our evaluations show that our distributed system running on underwater deployments of 4-5 commodity smart devices can perform pairwise ranging and localization with median errors of 0.5-0.9 m and 0.9-1.6 m

==> conclude.tex <==
%\section{Conclusion}

==> impl-1.tex <==





\section{Implementation and Evaluation}



Our ranging system has been implemented to run in the user space on Android devices. Our implementation performs the cross-correlation, auto-correlation and channel estimation algorithm within an average runtime of 90.1 ± 11.2~ms over a 500~ms audio sample buffer. We use the fftw3 library to perform FFTs in realtime. We use the OpenSL ES audio interface on Android which provides low-level access to the speaker and microphone audio buffers. In our system, the replying phone is configured to send a reply, one second after it has detected a preamble from the sender.  %Low-level access to the speaker buffer is required to send a reply at this precise delay time. We use the \textit{Overflow Flag} which  is thrown when the previous \textit{CallBack} is still running and a new \textit{CallBack} interruption occurs, leading to data loss that breaks up the  data stream. We  set an audio buffer size of {21888} samples to guarantee that no overflow happens and the \textit{CallBack} function always finish before next \textit{CallBack}.



==> pre-1.tex <==

\section{AquaRanger}

We first present the characterization of the channel resulting from the water-proof case and  then describe our system.



\subsection{Multipath with water-proof case}\label{sec:case}
% \begin{figure}[t!]
%     \includegraphics[width=.45\textwidth]{./figs/case2 (9)}
%     \vskip -0.15in
% \caption{(a) Smartphone in plastic bag and waterproof pouch. (b) Roll, pitch, and yaw axes used for different smartphone orientations.}
% % \vskip -0.15in
% \label{fig:case_img}
% \end{figure}

% \begin{figure}[t!]
%     \includegraphics[width=.45\textwidth]{./figs/water}
%     \vskip -0.15in
% \caption{{\bf Acoustic channel of smartphone in waterproof pouch underwater.}}
% \label{fig:water}
% \end{figure}

We  explore the effects of water-proof cases on the acoustic channel. We perform in-air experiments by placing two phones 10~cm away in an open space with no nearby reflectors.  We experiment with two different case material as shown in Fig.~\ref{fig:case1}. We run three groups of experiments: the phones without case,  phones with the first case, and phones with the second case. The first phone sends a 100~ms OFDM symbol between 1--5~kHz to the second phone where we perform channel estimation.  Figs.~\ref{fig:case1}a-b show the estimated channel with and without the two different case materials. The plots show that while the direct path is the strongest without the case, the multipath profile looks a lot more atypical with the cases. This is despite the  devices being close to each other and not having a close-by reflector. In addition, different case  materials   lead to different  channels, which makes it hard to predict and compensate for the water-proof case  since the phone can move around a bit  within it.
 
 
%At each direction, Phone A sent a 100ms OFDM (1--5~kHz) symbol to Phone B and Phone apply channel estimation. Fig.~\ref{fig:case} (a) displays the estimated channel without case (yellow dot line) and the estimated channel with case 1 (blue line) at three directions. Fig.~\ref{fig:case} (b) displays the estimated channel without case (yellow dot line) and the estimated channel with case 2 (blue line) at three directions. Based on our observation, the waterproof cases mainly have 3 effects:

%(1) The waterproof case would attenuate the acoustic signal, and attenuation in Direction2 is most severe.

%(2) The waterproof case would affect the multi-path profiles for the acoustic channel, by introducing many atypical paths. These atypical paths may be caused by propagation paths through case material, and sound reverberation between the phone and inner bound of case. The distortion of multi-path profiles in Direction2 is most severe, where the direct path is much lower than the multi-paths. 

%(3) The waterproof case would introduce obvious directionality to the smart phone. When we compare the channels without case for each directions (6 yellow dot lines in the Fig.~\ref{fig:case}), we can find the channel profiles are quite similar. However, when we compare the channel with case1 or case2 in different directions, their amplitude and multi-paths are quite different. The channel in Direction1 is most similar to the original channel without case, while channel distortion at Direction2 is the largest.

%Based on the above experiments results, the water-proof case would distort acoustic channel, by attenuating the direct path, changing the multi-path profiles, and introducing directionality. In addition, different material of case and different directions would lead to different effect on the channel, which makes it hard to predict and compensate the water-proof case effect.

In addition to the in-air experiments, we also performed channel estimation underwater. We put the two phones with the first water-proof case into the water. The phones are separated by 20~m and are at a depth of 2~m in a 9~m deep water body. Fig.~\ref{fig:case1}c shows that the multi-path profile is  dense compared to the air scenario; the former is  affected by both the water-proof case and the severe underwater reflections. Further, the multipath profile has peaks that appear before the direct path due to noise and low SNR signals.  %All these factors would challenge our underwater ranging systems design.
%Even though the case effect in air and under water is not exactly the same, but the in-air experiment. the water-proof case would distort acoustic channel, by attenuating the direct path, changing the multi-path profiles, and introducing directionality. This will be very challenging 



